Undertrained Image Reconstruction for Realistic Degradation in Blind Image Super-Resolution

Most super-resolution (SR) models struggle with real-world low-resolution (LR) images. This issue arises because the degradation characteristics in the synthetic datasets differ from those in real-world LR images. Since SR models are trained on pairs of high-resolution (HR) and LR images generated by downsampling, they are optimized for simple degradation. However, real-world LR images contain complex degradation caused by factors such as the imaging process and JPEG compression. Due to these differences in degradation characteristics, most SR models perform poorly on real-world LR images. This study proposes a dataset generation method using undertrained image reconstruction models. These models have the property of reconstructing low-quality images with diverse degradation from input images. By leveraging this property, this study generates LR images with diverse degradation from HR images to construct the datasets. Fine-tuning pre-trained SR models on our generated datasets improves noise removal and blur reduction, enhancing performance on real-world LR images. Furthermore, an analysis of the datasets reveals that degradation diversity contributes to performance improvements, whereas color differences between HR and LR images may degrade performance. 11 pages, (11 figures and 2 tables)

==> chaps/02_keywords.tex <==
\begin{keywords}
Super-resolution, Dataset generation, Image degradation, Real-world image, Image reconstruction.
\end{keywords}


==> chaps/10_biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/ru.png}}]{Ru Ito} received the B.E. degree in information engineering from Chiba University, in 2024, where he is currently pursuing the M.E. degree in information science. His research interests include deep learning and computer vision.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/supatta_photo.jpg}}]{Supatta Viriyavisuthisakul} received
her Ph.D. in engineering
technology at Sirindhorn International
Institute of Technology
(SIIT), Thailand, and information
science in School of Information
Science, Japan Advanced Institute
of Science and Technology
(JAIST). 
She is lecturer in Department of Mathematics in Faculty of Science, King Mongkut's University of Technology Thonburi, Thailand.
Her research areas are information technology and machine
learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/kawamoto.png}}]{Kazuhiko Kawamoto} (Member, IEEE) received the B.E., M.E., and Ph.D. degrees from Chiba University, in 1997, 1999, and 2002, respectively. From 2002 to 2005, he was an assistant professor at Tokyo Institute of Technology. From 2005 to 2009, he was an associate professor at Kyushu Institute of Technology. He is currently a professor at the Graduate School of Informatics, Chiba University. His research interests include computer vision and deep learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/kera.pdf}}]{Hiroshi Kera} (Member, IEEE) received his B.E., M.E., and Ph.D. degrees in engineering and information science from the University of Tokyo, Japan, in 2015, 2017, and 2020, respectively. Since 2021, he has been working as an assistant professor at the Graduate School of Informatics (previously the Graduate School of Engineering) at Chiba University. His main research includes computer algebra, deep learning, and computer vision.
\end{IEEEbiography}

